NTIRE 2020 Challenge on Real-World Image Super-Resolution: Methods and Results

This paper reviews the NTIRE 2020 challenge on real world super-resolution. It focuses on the participating methods and final results. The challenge addresses the real world setting, where paired true high and low-resolution images are unavailable. For training, only one set of source input images is therefore provided along with a set of unpaired high-quality target images. In Track 1: Image Processing artifacts, the aim is to super-resolve images with synthetically generated image processing artifacts. This allows for quantitative benchmarking of the approaches \wrt a ground-truth image. In Track 2: Smartphone Images, real low-quality smart phone images have to be super-resolved. In both tracks, the ultimate goal is to achieve the best perceptual quality, evaluated using a human study. This is the second challenge on the subject, following AIM 2019, targeting to advance the state-of-the-art in super-resolution. To measure the performance we use the benchmark protocol from AIM 2019. In total 22 teams competed in the final testing phase, demonstrating new and innovative solutions to the problem.

==> results_bak.tex <==
\section{Challenge Results}

\begin{table*}[t]
	\centering%
		\input{tables/track1}%}
	\label{tab:track1}
	\caption{Challenge results for Track 1}
	%\vspace{0mm}
\end{table*}

\begin{table*}[t]
	\centering%
	\resizebox{1.01\textwidth}{!}{%
		\input{tables/track2}}
	\label{tab:track2}
	\caption{Challenge results for Track 2}
	\vspace{0mm}
\end{table*}

Before the end of the final test phase, participating teams were required to submit results, code/executables, and factsheets for their approaches.
From 292 registered participants in Track 1, 19 valid methods were submitted, stemming from 16 different teams. Track 2 had 251 registered participants, of which 15 valid methods were submitted from 14 different teams. Table~\ref{tab:track1} and~\ref{tab:track2} report the final results of Track 1 and 2 respectively, on the test data of the challenge. The methods of the teams that entered the final phase are described in Section~\ref{sec:methods} and the teams' members and affiliations are shown in Section~\ref{sec:affiliation}.

\subsection{Architectures and Main Ideas} 
Inspired by the results of the last challenge in AIM 2019~\cite{AIM2019RWSRchallenge} and on the success of recent approaches~\cite{lugmayrICCVW2019,manuelFS}, most top methods pursued a two step approach. The first step aims to learn a network that can transfer \emph{clean} images to the source domain. This network thus learns a degradation operator, adding the kind of noise and corruptions present in the source images. It is then used to generate paired training data for the second step, which involves learning the super resolution network itself. It is generally trained using pairs generated by first downscaling and then applying the learned degradation on images from the target domain set. Many works employed the DSGAN~\cite{manuelFS} framework from the winner of the AIM 2019 challenge~\cite{AIM2019RWSRchallenge} to learn the degradation operator in the first step.

Some of the top methods in this challenge proposed particularly notable alterations and extensions to the general idea described above for learning the degradation network. The AITA-Noah team (Sec.~\ref{sec:AITA-Noah}) employs an iterative approach for Track~1, alternating between learning the degradation and SR network. It also uses an explicit denoising algorithm and train a sharpening network to decrease the blurring effects from the former. Impressionism (Sec.~\ref{sec:Impressionism}) is the only team that aims to explicitly estimate the blur kernel in the image, for improved source data generation. For Track~2, it employs the KernelGAN~\cite{Bell19InternalGAN} for this purpose. It also aims to explicitly estimate the noise variance using source image patches. This approach led to superior sharpness and quality in the generated SR images for Track~2. There were also some alternative strategies proposed. In particular, the Samsung-SLSI-MSL team (Sec.~\ref{sec:Samsung-SLSI-MSL}) aim to train a robust SR network capable of handling different source domains by randomly sampling a variety of degradations during the training of the SR network.

For the Real-world Super-Resolution setting, the results in the challenge suggest that training strategy and careful degradation modelling is far more important than choice of SR architecture. For the latter, most top methods simply adopted popular architectures, such as the RRDB/ESRGAN~\cite{wang2018esrgan} and the RCAN~\cite{rcan}. Most methods also included adversarial and perceptual VGG losses, often based on the ESRGAN~\cite{wang2018esrgan} framework. Brief descriptions of the methods submitted from each team is given in Sec.~\ref{sec:methods}.

\subsection{Baselines}
We compare methods participating in the challenge with several baseline approaches.

\parsection{Bicubic}
Standard bicubic upsampling using MATLAB's \verb|imresize| function.

\parsection{RRDB PT}
The pre-trained RRDB \cite{wang2018esrgan} method, using the network weights provided by the authors. The network was trained with clean images using bicubic down-sampling for supervision. The only objective is the PSNR oriented L1 loss.

\parsection{RRDB and ESRGAN Supervised}
RRDB and ESRGAN networks~\cite{wang2018esrgan} that is fine-tuned in a fully supervised manner, by applying the synthetic degradation operation used in Track~1. The degradation was unknown for the participants. This method therefore serves as an upper bound in performance, allowing us to analyze the gap between supervised and unsupervised methods. We employ the source $\mathcal{X}_\text{train}$ and target $\mathcal{Y}_\text{train}$ domain train images respectively. Low-resolution training samples are constructed by first down-sampling the image using the bicubic method and then apply the synthetic degradation. The network is thus trained with real input and output data, which is otherwise inaccessible. As for previous baselines, the network is initialized with the pre-trained weights provided by the authors. Note that no supervised baseline is available for Track~2 since no ground-truth HR images exists.

\subsection{Results: Track 1}


Here we present the final results of the challenge. All experiments presented were conducted on the test set for the respective tracks.

\parsection{Human perceptual study} In Track 1 (table~\ref{tab:track1}) the team Impressionism achieves the best MOS score, with an $0.23$ improvement over the second-best result and performs better than the ESRGAN fully supervised. The second-best score is achieved by the Samsung-SLSI-MSL team, which is $0.07$ better than the third best. As verified by the visual results (see figure~\ref{fig:visuals_track_1}), deep SR approaches are sensitive to such high-frequency degradations, unless explicitly trained to handle them. While only one participant in AIM2019 challenge~\cite{AIM2019RWSRchallenge} explicitly modeled the training input domain~\cite{manuelFS}, almost all submitted methods did so for this challenge. To increase the input domain knowledge, team AITA-Noah also trained on validation and test data. As this is against the challenge rules, we had to exclude them from the rankings.

As opposed to the Real-World Super-Resolution Challenge AIM 2019~\cite{AIM2019RWSRchallenge}, this year the winner has surpassed the performance of ESRGAN Fully-Supervised in terms of MOS. This team fine-tunes the model using patches with real noise for each test image individually.


\parsection{Computed Metrics}
Already at the start of the challenge, it was clarified that the final evaluation will be performed by a human study. We report PSNR, SSIM for reference. From the results it is clear that the participating methods did not optimize for fidelity only. It is noteworthy that the best performing method in terms of MOS/MOR (Impressionism) provides significantly worse PSNR and SSIM scores compared to all other participants. This suggest that the Impressionism team strongly focused on perceptual quality. It also confirms the limitations of the PSNR and SSIM metrics for perceptual evaluation, that were brought up by~\cite{ledig2017photo}.

We also report the learned LPIPS distance \cite{zhang2018unreasonable} for all approaches. It is a reference-based image quality metric, computed as the $L^2$ distance in a deep feature space, which is fine-tuned to correlate better with human perceptual opinions. Many methods employ feature-based losses using ImageNet pre-trained VGG networks, which in its design is very similar to LPIPS. Thus, although the LPIPS score seems to better correlate with MOS, it is difficult to draw any clear conclusions from this result. For Track 1, Impressionism achieves the best LPIPS and MOS, but there are differences in rank for the other nine of the top ten methods. In this track, the ESRGAN FT achieves a better LPIPS but a worse MOS than the challenge winner.

\parsection{Qualitative Analysis}
\label{parsec:quality}
Of the participating methods in Track 1, Impressionism achieves the visually most pleasing results as seen in Figure~\ref{fig:visuals_track_1}. Moreover this approach is able to almost completely remove the visible degradations. This is likely due to the degradation kernel estimation employed by Impressionism. The second rank goes to Samsung-SLSI-MSL, who made a SR network robust to noise, with data augmentation methods.

\subsection{Results: Track 2}

\parsection{Human perceptual study}
For Track 2 (table~\ref{tab:track2}), the Impressionism team also achieves the best MOR, with $1.54$ better than the second-best approch AITA-Noah-A. Which in turn was rated $0.26$ better than the third best. 


As opposed to the Real-World Super-Resolution Challenge AIM 2019~\cite{AIM2019RWSRchallenge}, this year the winner has surpassed the performance of ESRGAN Fully-Supervised in terms of MOS. This team fine-tunes the model using patches with real noise for each test image individually.

\parsection{Computed Metrics}
For track 2 a ground truth is non-existing due to the nature of the problem. Therefore we used several perceptual metrics. The NIQE, BRISQUE and PIQE as definded in Matlab, moreover the learned NRQM~\cite{MaYY017NRQM}. The Perceptual Index PI is calculated as an adjusted mean of NIQE and NRQM and the IQA-Rank is the average rank of the calculated metrics.

\parsection{Qualitative Analysis}
\label{parsec:quality}

Also in Track 2, the Impressionism team provides the visually most pleasing results as shown in Figures~\ref{fig:visuals_track_2_a}~and~\ref{fig:visuals_track_2_b}. Methods that use domain adaption were able to reduce the real-world super-resolution specific artifacts. As observed by~\cite{lugmayrICCVW2019}, CycleGAN can have problems with color shift. This effect can be observed in the visual example of MSMers. As shown in~\cite{AIM2019RWSRchallenge} methods with the approach of first cleaning the input~\cite{yuan2018unsupervised} have a very smooth super-resolution like KU-ISPL.


\begin{figure*}[t]
\centering
	\newcommand{\wid}{.195\linewidth}
	\newcommand{\im}[2]{
	\setlength\tabcolsep{-2pt}
    \begin{tabular}{c}
         \vspace{-4pt}
         \includegraphics[width=\wid]{figures/visuals/track1/0901/#1.png} \\
         \footnotesize{#2} %\tiny \scriptsize \footnotesize \small
    \end{tabular}}
    \im{Impressionism}{Impressionism}
    \im{Samsung_SLSI_MSL}{Samsung-SLSI-MSL}
    \im{BOE-IOT-AIBD}{BOE-IOT-AIBD}
    \im{MSMers}{MSMers}
    \im{KU_ISPL}{KU ISPL}
    \im{InnoPeak_SR}{InnoPeak-SR}
    \im{ITS425}{ITS425}
    \im{MLP_SR}{MLP-SR}
    \im{Webbzhou}{Webbzhou}
    \im{SR_DL}{SR-DL}
    \im{TeamAY}{TeamAY}
    \im{BIGFEATURE_CAMERA}{BIGFEATURE-CAMERA}
    \im{BMIPL_UNIST_YH_1}{BMIPL-UNIST-YH-1}
    \im{MLCV_SVNIT_NTNU_LAB}{SVNIT1-A}
    \im{KU-ISPL2}{KU-ISPL2}
    \im{SuperT}{SuperT}
    \im{GDUT-wp}{GDUT-wp}
    \im{MLCVLAB_SVNIT_NTNU}{SVNIT1-B}
    \im{MLDL_Lab_svnit_ntnu}{SVNIT2}
    \im{AITA_Noah_ExtraData}{AITA-Noah-A}
    \im{Noah_AITA_noExtraData}{AITA-Noah-B}
    \im{Bic}{Bic}
    \im{RRDB_FS}{RRDB Supervised}
    \im{ESRGAN_FS}{ESRGAN Supervised}
    \im{GT}{Ground Truth}\vspace{-0mm}
	\caption{Qualitative comparison between the challenge approaches for Track 1.  ($4\times$ super-resolution)}\vspace{-3mm}
	\label{fig:visuals_track_1}
\end{figure*}

\begin{figure*}[t]
\centering
	\newcommand{\wid}{.16\linewidth}
	\newcommand{\im}[2]{
	\setlength\tabcolsep{-2pt}
    \begin{tabular}{c}
         \vspace{-4pt}
         \includegraphics[width=\wid]{figures/visuals/track2/0/#1.png} \\
         \scriptsize{#2} %\tiny \scriptsize \footnotesize \small
    \end{tabular}}
    \im{Impressionism}{Impressionism}
    \im{AITA_Noah_ExtraData}{AITA-Noah-A}
    \im{ITS425}{ITS425}
    \im{Noah_AITA_noExtraData}{AITA-Noah-B}
    \im{Webbzhou}{Webbzhou}
    \im{Relbmag_Eht}{Relbmag-Eht}
    \im{MSMers}{MSMers}
    \im{MLP_SR}{MLP-SR}
    \im{SR_DL}{SR-DL}
    \im{InnoPeak_SR}{InnoPeak-SR}
    \im{QCAM}{QCAM}
    \im{SuperT}{SuperT}
    \im{KU_ISPL}{KU-ISPL}
    \im{BMIPL_UNIST_YH_1}{BMIPL-UNIST-YH-1}
    \im{BIGFEATURE_CAMERA}{BIGFEATURE-CAMERA}
    \im{Samsung_SLSI_MSL}{Samsung-SLSI-MSL}
    \im{Bic}{Bicubic}
    \im{RRDB}{RRDB Pre-trained}\vspace{1mm}
	\caption{Qualitative comparison between the challenge approaches for Track 2. ($4\times$ super-resolution)}\vspace{1mm}
	\label{fig:visuals_track_2_a}
\end{figure*}

\begin{figure*}[t]
\centering
	\newcommand{\wid}{.16\linewidth}
	\newcommand{\im}[2]{
	\setlength\tabcolsep{-2pt}
    \begin{tabular}{c}
         \vspace{-4pt}
         \includegraphics[width=\wid]{figures/visuals/track2/3/#1.png} \\ % Mercedes was track2/1/
         \scriptsize{#2} %\tiny \scriptsize \footnotesize \small
    \end{tabular}}
    \im{Impressionism}{Impressionism}
    \im{AITA_Noah_ExtraData}{AITA-Noah-A}
    \im{ITS425}{ITS425}
    \im{Noah_AITA_noExtraData}{AITA-Noah-B}
    \im{Webbzhou}{Webbzhou}
    \im{Relbmag_Eht}{Relbmag-Eht}
    \im{MSMers}{MSMers}
    \im{MLP_SR}{MLP-SR}
    \im{SR_DL}{SR-DL}
    \im{InnoPeak_SR}{InnoPeak-SR}
    \im{QCAM}{QCAM}
    \im{SuperT}{SuperT}
    \im{KU_ISPL}{KU-ISPL}
    \im{BMIPL_UNIST_YH_1}{BMIPL-UNIST-YH-1}
    \im{BIGFEATURE_CAMERA}{BIGFEATURE-CAMERA}
    \im{Samsung_SLSI_MSL}{Samsung-SLSI-MSL}
    \im{Bic}{Bicubic}
    \im{RRDB}{RRDB Pre-trained}\vspace{1mm}
	\caption{Qualitative comparison between the challenge approaches for Track 2. ($4\times$ super-resolution)}\vspace{1mm}
	\label{fig:visuals_track_2_b}
\end{figure*}

